Towards Flexible Inductive Bias via Progressive Reparameterization Scheduling

There are two de facto standard architectures in recent computer vision: Convolutional Neural Networks (CNNs) and Vision Transformers (ViTs). Strong inductive biases of convolutions help the model learn sample effectively, but such strong biases also limit the upper bound of CNNs when sufficient data are available. On the contrary, ViT is inferior to CNNs for small data but superior for sufficient data. Recent approaches attempt to combine the strengths of these two architectures. However, we show these approaches overlook that the optimal inductive bias also changes according to the target data scale changes by comparing various models' accuracy on subsets of sampled ImageNet at different ratios. In addition, through Fourier analysis of feature maps, the model's response patterns according to signal frequency changes, we observe which inductive bias is advantageous for each data scale. The more convolution-like inductive bias is included in the model, the smaller the data scale is required where the ViT-like model outperforms the ResNet performance. To obtain a model with flexible inductive bias on the data scale, we show reparameterization can interpolate inductive bias between convolution and self-attention. By adjusting the number of epochs the model stays in the convolution, we show that reparameterization from convolution to self-attention interpolates the Fourier analysis pattern between CNNs and ViTs. Adapting these findings, we propose Progressive Reparameterization Scheduling (PRS), in which reparameterization adjusts the required amount of convolution-like or self-attention-like inductive bias per layer. For small-scale datasets, our PRS performs reparameterization from convolution to self-attention linearly faster at the late stage layer. PRS outperformed previous studies on the small-scale dataset, e.g., CIFAR-100.

==> table/conv2vit.tex <==
\begin{table}[t]
\centering
\begin{tabular}{c|cccccc}
\toprule
Model & Ratio  & Acc@1 & Acc@5 & MaxAcc@1 & Flops & params \\ \midrule

\multirow{5}{*}{ConViT\_Tiny} & 0.01 & 6.08 & 15.824 & 6.1 & & \multirow{5}{*}{6M} \\
& 0.05	&26.934	& 49.86	& 26.98 & & \\
& 0.1	&42.918	&67.778	&42.99 &&\\
&0.5	&68.212	&88.934	&68.22 &&\\
&1	&73.1	&91.7 && \\ \midrule

\multirow{5}{*}{ResNet18} 
&0.01	&300	&13.928	&30.848		&&\multirow{5}{*}{1.8G}	&\multirow{5}{*}{11.6M} \\
&0.05	&300	&42.044	&67.582 & & \\			
&0.1	&300	&52.242	&76.38	& & \\
&0.5	&300	&66.38	&87.304	& & \\		
&1	&300	&69.528	&89.082 & & \\ \midrule

\multirow{5}{*}{ResT\_light} 
&0.01	&300	&11.19	&26.542	&11.38	&\multirow{5}{*}{1.4G}	 &\multirow{5}{*}{11M} \\
&0.05	&300	&42.922	&67.905	&43.2 & & \\		
&0.1	&258	&52.88	&76.618	&52.97 & & \\		
&0.5	&300	&73.028	&91.385	&73.16 & & \\		
&1	&300	&77	&93.6	&77.23 & & \\ \midrule

\multirow{4}{*}{DeiT-Tiny}
&0.01	&300	&6.426	&16.372	&6.426 & & \\
&0.05	&300	&24.82	&46.4	&24.98 & & \\
&0.1	&300	&38.61	&63.26	&38.66 & & \\
&0.5	&300	& ~ &	&	& \\ \midrule

\multirow{4}{*}{CanViT} 
&0.01	&294	&6.526	&16.12	&6.53 &
&\multirow{4}{*}{\makecell{28M $\rightarrow$ \\ 150M }} \\
&0.05	&294	&21.42	&41.45	&21.43 & & \\
&0.1	&294	&43.654	&67.59	&43.7 & & \\
&0.5	&294	&74.074	&91.602	&74.1 & & \\ \midrule


\multirow{5}{*}{Swin-Tiny}  
&0.01	&300	&13.2	&27.386	&13.35	&\multirow{5}{*}{4.5G}	&\multirow{5}{*}{28M} \\
&0.05	&300	&38.688	&61.88	&38.82 & & \\		
&0.1	&300	&53.464	&75.568	&53.47	& & \\	
&0.5	&300	&76.206	&92.864	&76.29	& & \\	
&1	&300	&81.2	&95.5	&-	& &  \\ 

\bottomrule




\end{tabular}
\caption{Caption}
\label{tab:my_label}
\end{table}

==> table/interpolation.tex <==
\begin{table}[!t]
\caption{Interpolation table.}
\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\small
\begin{tabular}{M{0.2\linewidth}|M{0.1\linewidth}
M{0.1\linewidth}M{0.1\linewidth}M{0.1\linewidth}}

\toprule
 \makecell{Reparam. \\Strategy} & Acc@1 & Acc@5 & Flops & \# params \\ \midrule

 50-250		&47.33	&xxxxx  & xxx & xxx \\ 

 150-150	&45.62	&68.88  & xxx & xxx \\

250-50	&44.29	&67.52 & xxx & xxx \\

300-0	&????   &xxxx	& xxx & xxx  \\
\bottomrule

\end{tabular}
\label{tab:interpolation}
\end{table}

==> table/main_imagenet_subset_2.tex <==
\begin{table}[!t]
\caption{\textbf{Data scale experiment of various model architectures}}

\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\small
\begin{tabular}{M{0.1\linewidth}|M{0.1\linewidth}M{0.1\linewidth}M{0.1\linewidth}M{0.15\linewidth}||M{0.1\linewidth}M{0.15\linewidth}}

\toprule
\makecell{ImgNet \\Ratio} & DeiT & ConViT & ResT & ResNet-18 & Swin & ResNet-50 \\ \midrule

0.01 & 6.426 & 6.08 & 11.19 & \textbf{13.928} & 13.2 & \textbf{13.668} \\
0.05 & 24.82 & 26.934 & \textbf{42.922} & 42.044  & 38.688  & \textbf{46.824} \\
0.1 & 38.61 & 42.918 & \textbf{52.88} & 52.242 & 53.464 & \textbf{58.142} \\
0.5 &  & 68.212 & \textbf{73.028} & 66.38 & \textbf{76.206} & 75.228 \\
1 & 72.2 & 6.426 & \textbf{73.1} & 69.528  & \textbf{81.2} & 80.152 \\ \midrule
Params & 5M & 6M  & 11M & 11.6M  & 28M & 23.9M \\
Flops & 1.25G & 1G & 1.4G & 1.8G  & 4.5G & 3.6G \\
% \multirow{5}{*}{0.01} 
% &ResNet-18	&\textbf{13.928} & \textbf{30.848}  &1.8G	&11.6M \\
% &DeiT-Tiny 	&42.044 & 67.582 & & \\			
% &ResT-light	&52.242 & 76.38	& & \\
% &ResNet-50	&66.38 &87.304	& & \\		
% &Swin-Tiny 	&69.528 & 89.082 & & \\ \midrule

% \multirow{5}{*}{0.05}
% &ResNet-18	&6.426	&16.372 &\multirow{5}{*}{1.25G}	 &\multirow{5}{*}{5M} \\
% &DeiT-Tiny 	&24.82	&46.4 & & \\
% &ResT-light	&38.61	&63.26 & & \\
% &ResNet-50	& ~ 	&	& & \\
% &Swin-Tiny       & 72.2  &   & & \\ \midrule

% \multirow{5}{*}{0.1} 
% &ResNet-18	&11.19	&26.542	&\multirow{5}{*}{1.4G}	 &\multirow{5}{*}{11M} \\
% &DeiT-Tiny 	&\textbf{42.922}	&\textbf{67.905} & & \\		
% &ResT-light	&52.88	&\textbf{76.618} & & \\		
% &ResNet-50	&73.028	&91.385 & & \\		
% &Swin-Tiny 	&77	&93.6 & & \\ \midrule

% \multirow{5}{*}{0.5} 
% &ResNet-18	&13.668 & 30.188 &\multirow{5}{*}{3.6G}	&\multirow{5}{*}{23.9M} \\
% &DeiT-Tiny 	&46.824 & 70.846 & & \\			
% &ResT-light	&58.142 & 80.53	& & \\
% &ResNet-50	&75.228 &92.416	& & \\		
% &Swin-Tiny 	&80.152 & 94.486 & & \\ \midrule

% \multirow{5}{*}{1}  
% &ResNet-18	&13.2	&27.386	&\multirow{5}{*}{4.5G}	&\multirow{5}{*}{28M} \\
% &DeiT-Tiny 	&38.688	&61.88 & & \\		
% &ResT-light	&\textbf{53.464}	&75.568	& & \\	
% &ResNet-50	&\textbf{76.206}	&\textbf{92.864}	& & \\	
% &Swin-Tiny 	&\textbf{81.2}	&\textbf{95.5}	& &  \\  

% \multirow{4}{*}{Ours} 
% &0.01	&294	&6.526	&16.12	&6.53 &
% &\multirow{4}{*}{\makecell{28M $\rightarrow$ \\ 150M }} \\
% &DeiT-Tiny 	&294	&21.42	&41.45	&21.43 & & \\
% &0.1	&294	&43.654	&67.59	&43.7 & & \\
% &0.5	&294	&74.074	&91.602	&74.1 & & \\
\bottomrule
\end{tabular}
 \vspace{-10pt}
\label{tab:main_imagenet}
\end{table}
